FinTral: A Family of GPT-4 Level Multimodal Financial Large Language Models

We introduce FinTral, a suite of state-of-the-art multimodal large language models (LLMs) built upon the Mistral-7b model and tailored for financial analysis. FinTral integrates textual, numerical, tabular, and image data. We enhance FinTral with domain-specific pretraining, instruction fine-tuning, and RLAIF training by exploiting a large collection of textual and visual datasets we curate for this work. We also introduce an extensive benchmark featuring nine tasks and 25 datasets for evaluation, including hallucinations in the financial domain. Our FinTral model trained with direct preference optimization employing advanced Tools and Retrieval methods, dubbed FinTral-DPO-T&R, demonstrates an exceptional zero-shot performance. It outperforms ChatGPT-3.5 in all tasks and surpasses GPT-4 in five out of nine tasks, marking a significant advancement in AI-driven financial technology. We also demonstrate that FinTral has the potential to excel in real-time analysis and decision-making in diverse financial contexts. The GitHub repository for FinTral is available at \url{https://github.com/UBC-NLP/fintral}.

==> error_analysis.tex <==
\section{Error Analysis} \label{error}

\subsection{Hallucination in LLMs}

One of the biggest dangers of using LLMs in the financial domain is their tendency to hallucinate or to give wrong answers or misinterpret things that are straightforward for a normal human being. As shown by \citep{kang2023deficiency} LLMs, including GPT-4 are prone to hallucinating basic facts. We created a dataset to evaluate how prone our models are to hallucinate. We have used the data generation method given by \citep{ghosh-EtAl:2022:FNP} to generate an evaluation dataset that contains terms and their definitions as we would like to evaluate how strong the financial basics of LLMs evaluated in this paper. We would also like to see if Retrieval-based methods can reduce hallucinations in our models. Examples of our evaluation dataset are in the appendix. This also serves as validation to see how well our model performs. 

We built a simple dataset to see if LLMs know basic financial definitions and if they can give the correct definition of the term we asked about. We created a dataset of 1129 terms. Some of them are highly technical, whereas others are trivial. 

==> tables/ZS_data.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\scriptsize
\begin{tabular}{lrrr}\toprule
Dataset &Categories &Number of Rows \\\midrule
IT risk disclosure &13 &1,200 \\
Firm Social Relationships &4 &4000 \\
Cyber Strategies &5 &200 \\
\bottomrule
\end{tabular}
\end{table}

==> tables/algo.tex <==
\begin{algorithm*}
\caption{Model Flow with Image and Retrieval Token Handling}
\begin{algorithmic}[1]
\State \textbf{Input:} \texttt{[INST] Human: [Instructions] [Task Input] <image> [Image Related Query] <retrieve> [Retrieved Task Relevant Input] [/INST]}
\State \textbf{Output:} Standard or with Operation Tools Tokens

\Procedure{HandleInput}{$input$}
    \If{\texttt{[Task Input]} is present}
        \State Process \texttt{[Task Input]}
    \EndIf
    \If{\texttt{<image>} tag is present}
        \State Use CLIP model for \texttt{[Image Related Query]}
        \State Obtain image embeddings
    \EndIf
    \If{\texttt{<retrieve>} tag is present}
        \State Retrieve documents from SEC filings
        \State Use text embedding models for relevance
    \EndIf
\EndProcedure

\end{algorithmic}
\end{algorithm*}

==> tables/prompt.tex <==
\begin{table}[h]
\centering
\begin{tabular}{|p{15cm}|}
\toprule
\textbf{Formatted Output for Multiple Inputs and Operation Tools Tokens} \\ 
\midrule
\textbf{Input:} \\
\texttt{[INST] Human: [Instructions] [Task Input]<image> [Image Related Query] <retrieve> [Retrieved Task Relevant Input] [/INST]}
\midrule
% \textbf{Standard Output:} \\
% \texttt{Assistant: [Output]} \\
% \midrule
% \textbf{Output with Operation Tools Tokens:} \\
% \texttt{Assistant: [Output] <add> [Additional Calculation] <multiply> [Multiplication Calculation]} \\
% \midrule
% \textbf{Output with Plot Token:} \\
% \texttt{Assistant: [Output] <plot> [Data for Plotting]} \\
\bottomrule
\end{tabular}
\caption{Prompt Format Table Demonstrating Multiple Input Handling and Operation Tools Token Output, Including Plotting}
\end{table}
